Digital Product Passport Management with Decentralised Identifiers and Verifiable Credentials

Digital product passports (DPP) have been proposed in the European Ecodesign for Sustainable Products Regulation (ESPR) as a means to keep and provide product information that facilitates product reusage, reparation, and recycling. Thus, DPPs should provide a positive effect on the environmental impact of future manufactured products, preventing waste and promoting a circular economy (CE) model. ESPR settles a set of requirements in collecting and administering product-related data. Decentralised identifiers (DID) and verifiable credentials (VC) are two self-sovereign-identity-related elements that may help in that DPP management since they introduce a decentralised administration of identity that may enhance the overall scalability of the resulting system, improving also its reliability. This paper analyses the ESPR requirements and describes how they may be achieved using DIDs and VCs, assessing their performance in some scenarios.

==> sec/productos.tex <==
Gafas ciclismo:

- Cristales: 
Cristales fotocromáticos categoría 1-3: filtran entre un 15 y un 55 % de la luz a 23 °C.
Con tiempo frío (menos de 10 °C) el cambio del tinte se vuelve más lento.
Norma ISO 12312-1.
Filtro 100% ANTI UV.

- Montura: 
Material de la montura: poliamida.
Material de los protectores del puente: caucho.
Material de las patillas: poliamida + caucho.
Material de los extremos de las patillas: caucho.


Ratón:

Externos:
- Armazón. plastic
- Botones. plastic
- Rueda. Rubber
- Tornillos. metal
- Almohadillas. rubber

Internos:
- Luz LED
- Prisma. plastic
- Sensor CMOS
- Microswitches. metal, plastic
- rotary encoder
- the circuit board. plastic, metal, and bits of silicon

==> sec/proposalOld.tex <==
TO DO: THIS SECTION SHOULD BE REWRITTEN COMPLETELY!!

The two examples of DPP management architecture based on DIDs described in Section \ref{solutions} make it clear that the use of DIDs and VCs in a system that maintains, administers, and enables the use of DPPs is feasible. However, the regulatory proposals related to DPPs, as described in Section \ref{normative}, would render their use impossible. Therefore, it might be possible to implement a pilot system to demonstrate the viability of this alternative with the goal of accommodating DIDs in the final wording of these regulations, allowing for more flexibility in product identification in DPPs. However, this would only make sense in a research project funded by the European Commission, whose results the Commission might consider. In another context, it would have little meaning. There are also some technical difficulties to consider:

\begin{enumerate}
    \item The recommendation (which, for practical purposes, can be considered a standard) from W3C related to decentralized identifiers (DID) \cite{Sporn22} appears to have stabilized in its version 1.0. Its specification was initiated on November 7, 2019, and the final draft was published on July 19, 2022. At present, there are no new drafts in progress for future versions. However, for the metasystem of digital identity management to function, verifiable credentials may also be required. The W3C specification for verifiable credentials has gone through several stages to reach a stable version 1.1, starting on August 3, 2017, with multiple drafts and the release of version 1.0 on November 19, 2019. It underwent a first revision on November 9, 2021, which generated version 1.1, and had another minor revision to create a new version 1.1 on March 3, 2022 \cite{Sporn22}. Following this, in August 2022, a new sequence of drafts was initiated to produce another version soon, version 2.0 \cite{Sporn23} which is still in progress. These specifications would need to be carefully analyzed, and if it is deemed advisable to use credentials to implement the DPP, those core features that do not require a redesign and new implementations and deployments should be used when the VC recommendation 2.0 stabilizes.
    \item To reduce the costs of issuance and management of DIDs and DPPs, it would be interesting to use permissioned blockchains instead of public ones to maintain the VDRs that will support the DID method (or methods) to be used in the proposed DPP management system. Remember that most public blockchains require fees for accepting each new transaction, thereby reducing profit margins for manufacturers or any other organizations that should collaborate in DPP management. Additionally, public blockchains typically employ consensus algorithms based on proof of work, which often require a high energy cost to achieve consensus. This energy cost would be contrary to the primary goal of DPPs: environmental sustainability in manufacturing processes. The specifications for DIDs and VCs are open to the use of various mechanisms and agent interaction protocols. Therefore, interoperability should be possible, regardless of the technologies used to implement VDRs. However, the uncertainty regarding which protocol and version will be necessary for various agent interactions could complicate their development and deployment.
    \item DIDs were proposed with the assumption that they would identify active subjects capable of initiating and conducting interactions with other entities. However, most products generated by the industry, whether in the European context or elsewhere, are passive entities that rarely initiate interactions voluntarily. Consequently, products may have an identifier, but they seldom require a pair of public and private keys to certify their identity. This characteristic complicates the assignment of VCs to a product and necessitates the involvement of another (active) entity to act as a controller of the DID for that passive product. Careful consideration is needed to determine which agent will assume this control role, avoiding overburdening.
    \item In any self-sovereign identity design, it is assumed that each entity to be identified can generate as many identifiers as they consider necessary to preserve privacy and avoid correlation in their various interactions with other entities. In other words, to some extent, the identified subject can create the specific identifier (the last component in the URI that constitutes the DID) for each of their DIDs. However, in the context of DPPs, this flexibility might not make much sense. Instead, each product should have a unique, public, and permanent identifier (although this does not preclude the internal storage of the identifiers of its potential multiple components by the DPP). As such, another entity is required to assign a specific identifier to each product or batch of products. Traditionally, this has been the responsibility of the manufacturer, typically following the ISO/IEC-15459 standard in case the product is labeled with a barcode. Therefore, it would be advisable to determine what name the DID method (or methods) used in the digital passport products will have and who will manage it. Since these products are passive entities, and their specific identifier in these methods need not be based on any public key, it seems like a good idea to maintain the ISO/IEC-15459 identifier as the specific identifier, as it has traditionally been used by the same manufacturing company to label each unit or batch of its products.
    \item Products manufactured in different industrial sectors may have very different characteristics. These characteristics will influence the content and granularity of the DPPs. It may be appropriate to distinguish three cases:
    \begin{itemize}
        \item Products with trivial or non-recyclable components: These are simple products with few components, low cost, and materials that pose no risk of pollution or contamination. There would be no need to manage a DPP for these types of products. Owners can simply deposit them in the most suitable container at the end of their useful life.
        \item Products with simple recycling: These products consist of a few parts and have a low or moderate total cost. Their affordability eliminates the need for repairs or replacements during their useful life. In this case, associating a DPP with each manufactured unit would not be necessary. A DPP for the complete model or reference would suffice. Since component replacement doesn't make sense, all manufactured units would have the same composition at the end of their useful life. The corresponding recycling center would only need to access common information about all these units to determine which part(s) should be recycled and how.
        \item Products with complex recycling: These are complex products consisting of multiple potentially hazardous components and with a high total cost. Due to their high cost and the existence of multiple components, in the event of a malfunction (or even periodically, as may occur in automobiles and motorcycles), the condition of these components must be reviewed, and those in need of replacement should be identified for recycling those that have reached the end of their useful life. In these cases, a DPP would be required for each manufactured unit. Typically, this DPP would have a hierarchical structure that includes the DPPs of the components that make up the product. Each of these DPPs would correspond, in turn, to a product with complex or simple recycling, depending on the case.
    \end{itemize}
\end{enumerate}

Following the analysis conducted in this document, some general recommendations may be made:

\begin{itemize}
    \item Products with simple recycling could have one DID per model, maintaining all information related to the composition of that model in the DID document. Although the DID document is a structure that holds certain metadata of the entity (initially designed to maintain at least the public keys and access points to the corresponding service), the W3C specification \cite{Sporn22} allows for other information to be stored within it. Therefore, it would be advisable to establish (and document in a new specification, even if unofficial) what attributes could be included in that document regarding the product's composition and the parts that can or should be recycled and the reasons for it.
    \item Products with complex recycling should have one DID per unit. The composition of each recyclable piece should be documented using VCs, as suggested by Guth-Orlowski in her articles \cite{Guth21, Guth22, Guth23}. Although the author does not document this in her work, it will require the creation of specific VC schemas that describe the structure that VCs should have, following the guidelines outlined in Section 5.4 (Data Schemas) of the VC specification \cite{Sporn22b}. However, this section is extremely brief and does not document how a schema should be structured or what fields it should contain. Therefore, a complementary specification has recently been initiated to address these aspects. As it can be observed, VC specifications are still evolving, which could complicate the development of a solution based on these tools.
\end{itemize}
